Profinite properties of residually free groups

Henry Wilton classified when a prime three-manifold $M$ has a residually free fundamental group $\pi_1 M$. We prove that the groups $\pi_1 M\times \mathbb Z^n$ are profinitely rigid within finitely generated residually free groups. We also establish other profinite invariants of the class of residually free groups such as coherence and subgroup separability. In the course of our proofs, we generalise a lemma of Wilton and Zalesskii on profinitely recognising when a central extension of groups splits.

==> report.tex <==
\begin{itemize}
    \item Now Theorem 3.2 has been corrected, "prime compact" has been replaced by "closed irreducible", as in Thm A. The closed assumption is important to ensure the three-manifold group is  PD3. 
    \item Either add orientable or deal with non-orientable PD3 or PD2 groups (and hence the involved surfaces may be non-orientable). But most examples from Wilton are non-orientable, so we should stick to this generality.
    \item We modified all long arrows $\lrar$ by shorter arrows $\rar$, which displays in a better way all our short exact sequences. 
    \item The mention on $K$ being finitely generated is now added, and it is precised Serre's reference with a section rather than with a page (which I think makes it easier to identify). We also corrected the cite from Serre's book on Lemma 3.3 (current labelling). 
    \item Added Lemma 3.1 to explain how to recognise whether a short exact sequence splits from the profinite completion, and added to the bibliography the article of Jiming-Zixi as another instance where this principle is applied.
    \item In Lemma 3.3, we replaced the assumption of $\FP$ by $\FP_{\infty}( \Z)$ because it is more natural and we apply it for finite groups $K$ in Lemma 3.1.
\end{itemize}

1. Corrected. 
2. There is an argument right after, where we reference a proposition from the book of Ribes on Profinite graphs and groups.
3. Corrected. 
4. We added the requested remarks to make it more clear how we actually use the separability of all its finite-index sugbroups. 
5. We added a separate lemma, and a proof, for the version of the Wilton--Zalesskii lemma that we need (where the quotient group is not a surface group). Regarding the last comment on how exactly the article of Wilton [Wil21] is used, we added a extended remark and another reference where this argument is explain in more detail. 
6. Updated. 
